Judge the Judges: A Large-Scale Evaluation Study of Neural Language Models for Online Review Generation

We conduct a large-scale, systematic study to evaluate the existing evaluation methods for natural language generation in the context of generating online product reviews. We compare human-based evaluators with a variety of automated evaluation procedures, including discriminative evaluators that measure how well machine-generated text can be distinguished from human-written text, as well as word overlap metrics that assess how similar the generated text compares to human-written references. We determine to what extent these different evaluators agree on the ranking of a dozen of state-of-the-art generators for online product reviews. We find that human evaluators do not correlate well with discriminative evaluators, leaving a bigger question of whether adversarial accuracy is the correct objective for natural language generation. In general, distinguishing machine-generated text is challenging even for human evaluators, and human decisions correlate better with lexical overlaps. We find lexical diversity an intriguing metric that is indicative of the assessments of different evaluators. A post-experiment survey of participants provides insights into how to evaluate and improve the quality of natural language generation systems.

==> conclusion.tex <==
%Final remarks
\section{Conclusion}
\label{Conclusion}

In summary, our findings represent a preliminary foundation for proposing more solid and robust evaluation metrics for the evaluation of natural language generation. First, we find that in the context of judging individual documents, discriminative evaluators are not as realistic as word-overlap evaluators, w.r.t. how they correlate with a simulated Turing test (human evaluators).  That implies that adversarial accuracy might not be the optimal objective for natural language generation, if the goal is to generate individual documents that humans consider as real.  %Instead, a fake review that fools humans does not necessarily need to fool a machine that has seen everything.  Pushing too hard towards the boundary might swing the pendulum too far towards rare corner or unrealistic cases.  
As a result, simple LSTM models or attention models may generate surprisingly competitive results.  In contrast, GAN based models may more easily pass a Turing test on a bot level (when judgments are made on a system as a whole instead of on individual items), or in a conversational context.  That is, when the judges have seen enough examples from the same generator, the next example had better be somewhat different. 

Our results also suggest that when adversarial training is used, the selection of training examples must be done with caution.  We also find that when humans are distinguishing fake reviews from real ones, they tend to focus more on the usage of words, expressions, emotions, and other details. %may be more convincing than something that is just ``generally'' correct.  
This may affect the design of objectives for the next generation of natural language generation models. 

%We believe that our findings represent a preliminary foundation for proposing more solid and robust evaluation metrics for the evaluation of NLG output. In future work we plan to carry additional experiments where we include in the study a wider range of generative models and meta-discriminator architectures, and inspired by the current results we aim to suggest more robust evaluation metrics for assessing the quality of NLG.

In the future we plan to carry additional experiments to include a wider range of generative models and discriminator architectures, and inspired by the current results we aim to design more meaningful objectives for natural language generation.
